Auto-Encoding Scene Graphs for Image Captioning

We propose Scene Graph Auto-Encoder (SGAE) that incorporates the language inductive bias into the encoder-decoder image captioning framework for more human-like captions. Intuitively, we humans use the inductive bias to compose collocations and contextual inference in discourse. For example, when we see the relation `person on bike', it is natural to replace `on' with `ride' and infer `person riding bike on a road' even the `road' is not evident. Therefore, exploiting such bias as a language prior is expected to help the conventional encoder-decoder models less likely overfit to the dataset bias and focus on reasoning. Specifically, we use the scene graph --- a directed graph ($\mathcal{G}$) where an object node is connected by adjective nodes and relationship nodes --- to represent the complex structural layout of both image ($\mathcal{I}$) and sentence ($\mathcal{S}$). In the textual domain, we use SGAE to learn a dictionary ($\mathcal{D}$) that helps to reconstruct sentences in the $\mathcal{S}\rightarrow \mathcal{G} \rightarrow \mathcal{D} \rightarrow \mathcal{S}$ pipeline, where $\mathcal{D}$ encodes the desired language prior; in the vision-language domain, we use the shared $\mathcal{D}$ to guide the encoder-decoder in the $\mathcal{I}\rightarrow \mathcal{G}\rightarrow \mathcal{D} \rightarrow \mathcal{S}$ pipeline. Thanks to the scene graph representation and shared dictionary, the inductive bias is transferred across domains in principle. We validate the effectiveness of SGAE on the challenging MS-COCO image captioning benchmark, e.g., our SGAE-based single-model achieves a new state-of-the-art $127.8$ CIDEr-D on the Karpathy split, and a competitive $125.5$ CIDEr-D (c40) on the official server even compared to other ensemble models.

==> Auto-Encoding Scene Graphs for Image Captioning/experiments.tex <==
\section{Experiments}
\subsection{Datasets}
\noindent\textbf{MSCOCO.} MSCOCO 2014 captions dataset is applied to evaluate our proposed method. This dataset contains $82,783$, $40,504$ and $40,775$ images for training, validation and testing respectively for online testing. About 5 human labeled captions are assigned to each image in the training and validation set and the ground truth captions of testing set is not available. In this online testing, the images of training set and validation set (123,287 images) are used to train our model.

For offline testing and fair comparison with the other caption models, the standard split provided by~\cite{karpathy2015deep} is also used in our experiments. In this `Karpathy' split, the training set contains $113,287$ images, validation set and testing set both contain $5,000$ images. In this offline testing, only images in training set (113,287 images) are used to train the model. 

We use the following steps to pre-process the captions: 1).the texts are tokenized on white space; 2).all the words are changed to lower words; and 3).the words which appear less than 5 times are labeled as one same label `UNK'; 4).each caption is trimmed to a maximum of 16 words. After the pre-processing, we have a vocabulary of $10,369$ words. 

\noindent\textbf{Visual Genome~\cite{krishna2017visual}.} This dataset concludes abundant scene graph annotations, \eg relationships between object pairs and attributes of each object. Since this dataset is labeled by crowd workers and the annotations are very noisy, we only choose the relationships and attributes which appear more than $2,000$ times in the training set. After filtering, $64$ kinds of relationships and $103$ kinds of attributes are used to train our relationship and attribute classifiers. 

\subsection{Experiment Settings}
\noindent\textbf{Metrics.}
To evaluate the performance of the proposing model, four standard automatic evaluations which include CIDEr~\cite{vedantam2015cider}, BLEU~\cite{papineni2002bleu}, METEOR\cite{banerjee2005meteor} and ROUGE~\cite{lin2004rouge}, are used. 

\noindent\textbf{Comparing methods.} To quantify the importance of graph-level embeddings and the necessary of the complied dictionary, the proposed method is compared with he following ablative baselines:

\textbf{OE.} We directly reimplement the model described in~\cite{anderson2018bottom}, in which only object-level embeddings are used. 

\textbf{GE.} We do not compile a dictionary and only use the components in image branch.

\textbf{OE+DC.} The complied dictionary is used, but when generating captions from images, only object-level embeddings are used.

\textbf{DC w/o SG.} When compiling the dictionary, we do not use sentence GNN to create graph-level embeddings and only input the word embedding of each word in the caption to the self-translator.

\textbf{DC + I-SG.} In the image branch, the image GNN only use word embedding of nodes in predicted image scene graph instead of RoI features to create the graph-level embedding. The rest is not changed. 

We also compare our model with some state-of-the-art captioning models such as \textbf{SCST}~\cite{rennie2017self}, \textbf{Up-Down}~\cite{anderson2018bottom}, \textbf{GCN-LSTM}~\cite{yao2018exploring}, \textbf{StackCap}~\cite{gu2017stack}, \textbf{LSTM-A}~\cite{yao2017boosting} and \textbf{CAVP}~\cite{liu2018context}. 


\subsection{Results and Analysis}
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth,trim = 5mm 3mm 5mm 5mm,clip]{latex/fig_exp.pdf}
   \caption{}
\label{fig:fig_exp}
\end{figure*}
Table~\ref{table:tab_kap} shows the performance of proposed methods and compared models on COCO's Karpathy split. As we can see, compared with the vanilla baseline \textbf{OE}, the proposed method can boost the B@1, B@4, M, R, C, and S  by absolute $\cdot$, $\cdot$, $\cdot$, $\cdot$, $\cdot$, and $\cdot$ respectively on Karpathy split of COCO dataset.

By comparing \textbf{GE} with \textbf{OE}, and \textbf{DC} with \textbf{OE}, the performances of different metrics have certain improvements, which substantiate that the proposed graph-level embedding and dictionary compiling are both indispensable for advancing the performances. Also, it can be found that the boost of using \textbf{DC} is larger than using \textbf{GE}, which suggest that the introduction of humans' especial expressions plays a more significant role in generating human-like captions. 

It is noteworthy that for model \textbf{GCN-LSTM}~\cite{yao2018exploring}, their batch size is set to $1,024$ and they train the whole model about $250$ epochs. Due to the limitation of computation resources, we only set the batch size to $100$, which is the same as \textbf{CAVP}~\cite{liu2018context} and \textbf{Up-Down}~\cite{anderson2018bottom}, and the maximum epochs to 100. Since we also propose one kind of GNN, and for fair comparison, we reimplement their work (their code is not published) and report the result, which is denoted as \textbf{GCN-LSTM$_{re}$}.
Also, the best result reported by~\cite{yao2018exploring} is got by fusing two different predicted probabilities, one for semantic relationship and one for spatial relationship, by using manual chosen weights. In the table~\ref{table:tab_kap}, the result of single model and fusion model in~\cite{yao2018exploring} are denoted as  \textbf{GCN-LSTM$_{sem}$} and \textbf{GCN-LSTM$_{fuse}$}. For fair comparison, we also follow them to fuse two distributions got by using two kinds of relationships, and such result is denoted as \textbf{DC+GE}$_{fuse}$.

Table~\ref{table:tab_online} shows the performances on COCO online testing server. The result reported by~\cite{yao2018exploring} is not in the leaderboard of online testing website and we directly use the result reported in their literature. We submit two kinds of predicted results, one for single model (\textbf{DC+GE}) and one for fusion model (\textbf{DC+GE}$_{fuse}$).

\begin{table}[t]
\begin{center}
\caption{The performances of our DC+GE and the compared methods, including ablative baselines and other state-of-the-art captioning methods, on COCO's Karpathy split. The metrics: B@N, M, R, C and S refer to BLEU@N, METEOR, ROUGE-L, CIDEr-D and SPICE respectively. In all cases, the scores are reported as percentage ($\%$)}
\label{table:tab_kap}
\scalebox{0.78}{
\begin{tabular}{|c||c|c|c|c|c|c|}
		\hline
		   Metric   & B@1 & B@4 & M & R &  C & S\\ \hline
           \textbf{OE}       & $79.9$ & $36.8$& $27.7$ & $57.0$ & $120.6$ & $20.9$\\ \hline
           \textbf{GE}       & $80.2$ & $37.1$& $27.6$ & $57.5$ & $123.4$ & $21.2$\\ \hline
           \textbf{DC}       & $80.2$ & $37.5$& $28.0$ & $58.3$ & $124.5$ & $21.3$\\ \hline
           \textbf{DC+GE}    & $80.8$ & $38.4$ & $28.4$ & $58.6$ & $127.8$ & $21.8$\\ \hline 
           \textbf{DC+GE$_{fuse}$}    & $-$ & $-$ & $-$ & $-$ & $-$ & $-$\\ \hline \hline
           \textbf{SCST}~\cite{rennie2017self}       & $-$  & $34.2$ & $26.7$ & $55.7$ & $114.0$ & $-$   \\ \hline
           \textbf{LSTM-A}~\cite{yao2017boosting}   & $78.6$  & $35.5$ & $27.3$ & $56.8$ & $118.3$ & $20.8$   \\ \hline
           \textbf{StackCap}~\cite{gu2017stack}    & $78.6$  & $36.1$ & $27.4$ & $-$ & $120.4$ & $-$   \\ \hline
           \textbf{Up-Down}~\cite{anderson2018bottom}  & $79.8$ & $36.3$ & $27.7$ & $56.9$ & $120.1$ & $21.4$ \\ \hline
           \textbf{CAVP}~\cite{liu2018context}  & $-$& $38.6$ & $28.3$ & $58.5$ & $126.3$ & $21.6$ \\ \hline
           \textbf{GCN-LSTM$_{re}$}~\cite{yao2018exploring}  & $-$  & $-$ & $-$ & $-$ & $-$ & $-$ \\ \hline
           \textbf{GCN-LSTM$_{sem}$}~\cite{yao2018exploring}  & $80.5$  & $38.2$ & $28.5$ & $58.3$ & $127.6$ & $22.0$ \\ \hline
           \textbf{GCN-LSTM$_{fuse}$}~\cite{yao2018exploring} & $80.9$  & $38.3$ & $28.6$ & $58.5$ & $128.7$ & $22.1$ \\ \hline
           
\end{tabular}
}
\end{center}
\end{table}

\begin{table*}[t]
\begin{center}
\caption{The performances of our DC+GE and the compared methods, including ablative baselines and other state-of-the-art captioning methods, on online COCO testing set (\url{https://competitions.codalab.org/competitions/3221#results}). The metrics: B@N, M, R, C and S refer to BLEU@N, METEOR, ROUGE-L, CIDEr-D and SPICE respectively. In all cases, the scores are reported as percentage ($\%$)}
\label{table:tab_online}
\scalebox{0.93}{
\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		 %Model & \multicolumn{2}{|c|}{BLEU-1}  & \multicolumn{2}{|c|}{BLEU-2}  & \multicolumn{2}{|c|}{BLEU-3} & \multicolumn{2}{|c|}{BLEU-4} &\multicolumn{2}{|c|}{METEOR} &\multicolumn{2}{|c|}{ROUGE-L} & \multicolumn{2}{|c|}{CIDEr-D}\\ \hline
		 Model & \multicolumn{2}{|c|}{B@1}  & \multicolumn{2}{|c|}{B@2}  & \multicolumn{2}{|c|}{B@3} & \multicolumn{2}{|c|}{B@4} &\multicolumn{2}{|c|}{M} &\multicolumn{2}{|c|}{R-L} & \multicolumn{2}{|c|}{C-D}\\ \hline
		 Metric  &  c5 & c40 & c5 & c40 &  c5 & c40 & c5 & c40 & c5 & c40 & c5 & c40 & c5 & c40 \\ \hline
           %\textbf{OE}       & $76.8$ & $36.3$  & $27.3$ & $56.4$ & $114.3$  & $20.5$ & $79.9$ & $36.8$& $27.7$ & $57.0$ \\ \hline
           %\textbf{GE}       & $77.8$ & $36.3$  & $27.4$ & $56.6$ & $114.8$  & $20.5$ & $80.2$ & $37.1$& $27.6$ & $57.5$\\ \hline
           %\textbf{DC}       & $78.2$ & $36.4$  & $27.7$ & $56.7$ & $115.3$  & $20.7$ & $80.2$ & $37.5$& $28.0$ & $58.3$ \\ \hline
           \textbf{DC+GE}    & $80.6$ & $95.0$  & $65.0$ & $88.9$ & $50.1$  & $79.6$ & $37.8$ & $68.7$& $28.1$ & $37.0$ & $58.2$ & $73.1$ & $122.7$ & $125.5$\\ \hline 
           \textbf{DC+GE$_{fuse}$}    & $-$ & $-$  & $-$ & $-$ & $-$  & $-$ & $-$ & $-$& $-$ & $-$ & $-$ & $-$ & $-$ & $-$\\ \hline \hline
           \textbf{SCST}~\cite{rennie2017self}      & $78.1$ & $93.7$ & $61.9$ & $86.0$ & $47.0$ & $75.9$ & $35.2$ & $64.5$ & $27.0$ & $35.5$ & $56.3$ & $70.7$ & $114.7$ & $116.0$  \\ \hline
           \textbf{LSTM-A}~\cite{yao2017boosting}   & $78.7$ & $93.7$ & $62.7$ & $86.7$ & $47.6$ & $76.5$ & $35.6$ & $65.2$ & $27.0$ & $35.4$ & $56.4$ & $70.5$ & $116.0$ & $118.0$  \\ \hline
           \textbf{StackCap}~\cite{gu2017stack}     & $77.8$ & $93.2$ & $61.6$ & $86.1$ & $46.8$ & $76.0$ & $34.9$ & $64.6$ & $27.0$ & $35.6$ & $56.2$ & $70.6$ & $114.8$ & $118.3$   \\ \hline
           \textbf{Up-Down}~\cite{anderson2018bottom}    & $80.2$ & $95.2$ & $64.1$ & $88.8$ & $49.1$ & $79.4$ & $36.9$ & $68.5$ & $27.6$ & $36.7$ & $57.1$ & $72.4$ & $117.9$& $120.5$  \\ \hline
           \textbf{CAVP}~\cite{liu2018context}           & $80.1$ & $94.9$ & $64.7$ & $88.8$ & $50.0$ & $79.7$ & $37.9$ & $69.0$ & $28.1$ & $37.0$ & $58.2$ & $73.1$ & $121.6$& $123.8$    \\ \hline
            \textbf{GCN-LSTM$_{fuse}$}~\cite{yao2018exploring}           & $-$ & $-$ & $65.5$ & $89.3$ & $50.8$ & $80.3$ & $38.7$ & $69.7$ & $28.5$ & $37.6$ & $58.5$ & $73.4$ & $125.3$& $126.5$    \\ \hline
\end{tabular}
}
\end{center}
\end{table*}

\subsection{Enlightening Studies}
\textbf{Using Oracle Scene Graphs.}
In the sentence branch, the used sentence scene graphs are created by the ground truth captions. Then, suppose we have such kind of oracle scene graphs when inference, how better the generated captions can be? For exploring such a question, we generate sentence scene graphs by inputting the labeled captions, which belong to Karpathy's test set, into tools provided by~\cite{anderson2016spice}. Then we 1).directly feed the sentence graph embeddings to self-translator (route 1) to generate captions; 2).use sentence graph embeddings to consult the dictionary and then feed the consulted entries to self-translator (route 2) to generate captions. The results of different routes are shown in Table~\ref{table:tab_orac}. 

As we can see, the performances of using oracle sentence scene graphs (whether \textbf{Route 1} or \textbf{Route 2}) are far better than \textbf{DC+GE}. This is reasonable since the oracle sentence scene graphs contain almost no noises and are abundant in humans' descriptive expressions. By comparing \textbf{Route 1} and \textbf{Route 2}, we can see that directly using oracle sentence scene graphs would produce much better captions; and by comparing \textbf{Route 2} with \textbf{DC+GE}, we find that consulting dictionaries by oracle sentence scene graphs would generate more human-like captions. Both of these two observations encourage us to develop some more powerful techniques to compile and consult dictionary.

\begin{table}[t]
\begin{center}
\caption{The performances of using oracle sentence scene graphs}
\label{table:tab_orac}
\scalebox{0.88}{
\begin{tabular}{|c||c|c|c|c|c|c|}
		\hline
		   Metric   & B@1 & B@4 & M & R &  C & S\\ \hline
		   \textbf{DC+GE}    & $80.8$ & $38.4$ & $28.4$ & $58.6$ & $127.8$ & $21.8$\\ \hline
           \textbf{Route 1}  & $93.94$ & $65.21$& $38.51$ & $71.85$ & $177.0$ & $34.38$\\ \hline
           \textbf{Route 2}  & $90.38$ & $53.86$& $34.03$ & $66.53$ & $153.2$ & $30.69$\\ \hline
\end{tabular}
}
\end{center}
\end{table}

\textbf{Using Web Description Texts.}
There is a nearly unlimited amount of free description texts available in website, thus, if these resources can be rationally exploited, the performance of captioning model will naturally be improved. For discovering the potential ability of using web description texts in our model, we use the texts provided by Visual Genome~\cite{krishna2017visual} instead of COCO caption dataset~\cite{lin2014microsoft} to learn the dictionary in sentence branch. And then we follow route 3 to train image branch. The results is demonstrated in~\ref{table:tab_web}.
\begin{table}[t]
\begin{center}
\caption{The performances of using web description texts}
\label{table:tab_web}
\scalebox{0.95}{
\begin{tabular}{|c||c|c|c|c|c|c|}
		\hline
		   Metric   & B@1 & B@4 & M & R &  C & S\\ \hline
		   \textbf{OE}       & $79.9$ & $36.8$& $27.7$ & $57.0$ & $120.6$ & $20.9$\\ \hline
		   \textbf{Web}  & $-$ & $-$& $-$ & $-$ & $-$ & $-$\\ \hline
		   \textbf{DC+GE}    & $80.8$ & $38.4$ & $28.4$ & $58.6$ & $127.8$ & $21.8$\\ \hline
          
\end{tabular}
}
\end{center}
\end{table}

==> Auto-Encoding Scene Graphs for Image Captioning/intro.tex <==
%%%%%%%%% BODY TEXT
\section{Introduction}
For image captioning, there are two ingredients spurring its success: a visual system, which used as encoding module, should be able to accurately recognize the appeared visual clues; and one language system, which used as decoding module, should be able to compose these revealed clues to one human-like caption.

On the one hand, benefiting from the ingeniously designed deep networks, some fundamental computer vision tasks like classification, detection or segmentation have achieved unprecedented success. 
The fruits of these achievements are further extended to the image captioning task that these deep CNNs are usually used as encoding module to extract representations which are rich in visual clues.
For example, by exploiting a well pre-trained object detection network, Faster R-CNN~\cite{ren2015faster}, to seek the salient regions in one image, the generated captions now are more visual grounding to the images~\cite{anderson2018bottom}. Here, visual grounding means that the named concepts in one caption are associated to the objects appeared in one image~\cite{lu2018neural}.

On the another hand, in order to capture the intimate connection among a sentence, Long Short Term Memory (LSTM)~\cite{hochreiter1997long} is usually built as one decoding module to generate the caption. 
Also, for the sake of establishing closer ties between generated language with images, attention mechanisms of different usage~\cite{xu2015show,lu2017knowing,anderson2018bottom} are incorporated into the decoding systems. Though these mechanisms own diverse scheming details, the main role are similar that try to make the decoding module focus on some specific regions of the image conditioned on the sentence generated so far.
Furthermore, by applying reinforcement learning~\cite{rennie2017self} to optimize the whole system with sentence-level metric such as CIDEr metric~\cite{vedantam2015cider}, the generated captions are more likely to be fluent, well-formed compared with the system trained by cross-entropy loss.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth,trim = 5mm 3mm 5mm 5mm,clip]{latex/fig_intro.pdf}
   \caption{}
\label{fig:fig_intro}
\end{figure}

However, generating grounding and fluent captioning is only one small step in the long march of generating human-like caption. For one image, humans can not only recognize the salient objects along with their visual attributes (\ie colour, shape or size) to compose one description, but also associate these visual cues to some more complex or descriptive terms by common sense and life experiences. For example, as shown in Fig~\ref{fig:fig_intro}, human may describe `yellow banana' as `ripe banana' or describe `a room full with many items' as `cluttered room'. 

While some modern systems like~\cite{anderson2018bottom,lu2018neural} can hardly compose one caption with these descriptive or more human-like terms. There are two reasons which cause the model be difficult in capturing these more flexible terms.
1). These models usually use object-level embedding, \eg the RoI pooling of one object. Then, when generating next word, the language model usually only focuses on one object by predicting one attention distribution over these objects. Such object-level hinder the system from composing complex phrases since these kind of embeddings usually only contain the information about the categories of these objects or at most some additional visual attribute information. 
2). The second reason is that these systems are usually optimized by CIDEr, which is a consensus-based evaluation protocol that it prefers a description which owns more similarity to the majority reference captions. Then the caption system trends to provide overly general captions which only combines the appeared salient objects together as one grounding and fluent caption, while suppress the various and flexible descriptions about interesting details appeared in one image. 

For generating more human-like captions, we propose a captioning model which is trained by `Dictionary Compiling and Consulting' strategy. For `Dictionary Compiling', firstly, we use graph neural network to embed one sentence scene graph to sentence embeddings and recompose one sentence from these embeddings with a self-translator. In this stage, the sentence graph neural network and self-translator are trained. Then we compile one dictionary which should save these sentence embeddings. When compiling dictionary, we use these sentence embeddings as indexes to consult entries from the dictionary, and then feed these consulted entries into the self-translator to recompose the sentence. After compiling the dictionary, when generating one caption from one image, we use one image graph neural network to embed visual feature and then use them to consult the compiled dictionary to find corresponding entries. And the consulted entries and these visual embedding features are all feed into one caption generator to get the final caption. Here we use a differentiable operation to implement consulting, and thus the whole system can be trained end-to-end.

Compared with object-level embedding used in~\cite{lu2017knowing,lu2018neural,anderson2018bottom}, we use graph neural network to embed the triplet information like <subject-predicate-object> or <attribute-object> together. From the language perspective, object-level embedding corresponding to word-level expression and graph-level embedding corresponding to phrase-level expression.
By using attention mechanism to predict an attention distributions over these graph embeddings, the language system can incorporate more visual clues. Furthermore, the visual graph embedding is used to consult corresponding dictionary entries which contains abundant distinctive expressions. Both visual graph embedding and the consulted dictionary entries enable the language system to generate more human-like sentences.  

\textbf{Contributions:} Our contributions can be concluded as follows:
\begin{itemize}[nolistsep]
\item We propose the Dictionary Compiling and Consulting model, which can incorporate visual embeddings with more clues and phrase embeddings with distinctive expressions together to compose more human-like captions.
\item Graph neural network is used to embed scene graph information together to get graph-level embedding for image and sentence.
\item A dictionary which contains embeddings with abundant human-like expressions is compiled. When generating captions, this dictionary is consulted with visual graph embeddings as indexes to provide more complex and descriptive information for composing human-like descriptions.
\item Exhaust experiments show that our proposed method can achieve obvious improvements compared with baselines. Ablation studies are also designed to prove that each added component play certain roles in improving performance. 
\end{itemize}

==> experiments.tex <==
\section{Experiments}
\subsection{Datasets}
\noindent\textbf{MSCOCO.} MSCOCO 2014 captions dataset is applied to evaluate our proposed method. This dataset contains $82,783$, $40,504$ and $40,775$ images for training, validation and testing respectively for online testing. About 5 human labeled captions are assigned to each image in the training and validation set and the ground truth captions of testing set is not available. In this online testing, the images of training set and validation set (123,287 images) are used to train our model.

For offline testing and fair comparison with the other caption models, the standard split provided by~\cite{karpathy2015deep} is also used in our experiments. In this `Karpathy' split, the training set contains $113,287$ images, validation set and testing set both contain $5,000$ images. In this offline testing, only images in training set (113,287 images) are used to train the model. 

We use the following steps to pre-process the captions: 1).the texts are tokenized on white space; 2).all the words are changed to lower words; and 3).the words which appear less than 5 times are labeled as one same label `UNK'; 4).each caption is trimmed to a maximum of 16 words. After the pre-processing, we have a vocabulary of $10,369$ words. 

\noindent\textbf{Visual Genome~\cite{krishna2017visual}.} This dataset concludes abundant scene graph annotations, \eg relationships between object pairs and attributes of each object. Since this dataset is labeled by crowd workers and the annotations are very noisy, we only choose the relationships and attributes which appear more than $2,000$ times in the training set. After filtering, $64$ kinds of relationships and $103$ kinds of attributes are used to train our relationship and attribute classifiers. 

\subsection{Experiment Settings}
\noindent\textbf{Metrics.}
To evaluate the performance of the proposing model, four standard automatic evaluations which include CIDEr~\cite{vedantam2015cider}, BLEU~\cite{papineni2002bleu}, METEOR\cite{banerjee2005meteor} and ROUGE~\cite{lin2004rouge}, are used. 

\noindent\textbf{Comparing methods.} To quantify the importance of graph-level embeddings and the necessary of the complied dictionary, the proposed method is compared with he following ablative baselines:

\textbf{OE.} We directly reimplement the model described in~\cite{anderson2018bottom}, in which only object-level embeddings are used. 

\textbf{GE.} We do not compile a dictionary and only use the components in image branch.

\textbf{OE+DC.} The complied dictionary is used, but when generating captions from images, only object-level embeddings are used.

\textbf{DC w/o SG.} When compiling the dictionary, we do not use sentence GNN to create graph-level embeddings and only input the word embedding of each word in the caption to the self-translator.

\textbf{DC + I-SG.} In the image branch, the image GNN only use word embedding of nodes in predicted image scene graph instead of RoI features to create the graph-level embedding. The rest is not changed. 

We also compare our model with some state-of-the-art captioning models such as \textbf{SCST}~\cite{rennie2017self}, \textbf{Up-Down}~\cite{anderson2018bottom}, \textbf{GCN-LSTM}~\cite{yao2018exploring}, \textbf{StackCap}~\cite{gu2017stack}, \textbf{LSTM-A}~\cite{yao2017boosting} and \textbf{CAVP}~\cite{liu2018context}. 


\subsection{Results and Analysis}
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth,trim = 5mm 3mm 5mm 5mm,clip]{latex/fig_exp.pdf}
   \caption{}
\label{fig:fig_exp}
\end{figure*}
Table~\ref{table:tab_kap} shows the performance of proposed methods and compared models on COCO's Karpathy split. As we can see, compared with the vanilla baseline \textbf{OE}, the proposed method can boost the B@1, B@4, M, R, C, and S  by absolute $\cdot$, $\cdot$, $\cdot$, $\cdot$, $\cdot$, and $\cdot$ respectively on Karpathy split of COCO dataset.

By comparing \textbf{GE} with \textbf{OE}, and \textbf{DC} with \textbf{OE}, the performances of different metrics have certain improvements, which substantiate that the proposed graph-level embedding and dictionary compiling are both indispensable for advancing the performances. Also, it can be found that the boost of using \textbf{DC} is larger than using \textbf{GE}, which suggest that the introduction of humans' especial expressions plays a more significant role in generating human-like captions. 

It is noteworthy that for model \textbf{GCN-LSTM}~\cite{yao2018exploring}, their batch size is set to $1,024$ and they train the whole model about $250$ epochs. Due to the limitation of computation resources, we only set the batch size to $100$, which is the same as \textbf{CAVP}~\cite{liu2018context} and \textbf{Up-Down}~\cite{anderson2018bottom}, and the maximum epochs to 100. Since we also propose one kind of GNN, and for fair comparison, we reimplement their work (their code is not published) and report the result, which is denoted as \textbf{GCN-LSTM$_{re}$}.
Also, the best result reported by~\cite{yao2018exploring} is got by fusing two different predicted probabilities, one for semantic relationship and one for spatial relationship, by using manual chosen weights. In the table~\ref{table:tab_kap}, the result of single model and fusion model in~\cite{yao2018exploring} are denoted as  \textbf{GCN-LSTM$_{sem}$} and \textbf{GCN-LSTM$_{fuse}$}. For fair comparison, we also follow them to fuse two distributions got by using two kinds of relationships, and such result is denoted as \textbf{DC+GE}$_{fuse}$.

Table~\ref{table:tab_online} shows the performances on COCO online testing server. The result reported by~\cite{yao2018exploring} is not in the leaderboard of online testing website and we directly use the result reported in their literature. We submit two kinds of predicted results, one for single model (\textbf{DC+GE}) and one for fusion model (\textbf{DC+GE}$_{fuse}$).

\begin{table}[t]
\begin{center}
\caption{The performances of our DC+GE and the compared methods, including ablative baselines and other state-of-the-art captioning methods, on COCO's Karpathy split. The metrics: B@N, M, R, C and S refer to BLEU@N, METEOR, ROUGE-L, CIDEr-D and SPICE respectively. In all cases, the scores are reported as percentage ($\%$)}
\label{table:tab_kap}
\scalebox{0.78}{
\begin{tabular}{|c||c|c|c|c|c|c|}
		\hline
		   Metric   & B@1 & B@4 & M & R &  C & S\\ \hline
           \textbf{OE}       & $79.9$ & $36.8$& $27.7$ & $57.0$ & $120.6$ & $20.9$\\ \hline
           \textbf{GE}       & $80.2$ & $37.1$& $27.6$ & $57.5$ & $123.4$ & $21.2$\\ \hline
           \textbf{DC}       & $80.2$ & $37.5$& $28.0$ & $58.3$ & $124.5$ & $21.3$\\ \hline
           \textbf{DC+GE}    & $80.8$ & $38.4$ & $28.4$ & $58.6$ & $127.8$ & $21.8$\\ \hline 
           \textbf{DC+GE$_{fuse}$}    & $-$ & $-$ & $-$ & $-$ & $-$ & $-$\\ \hline \hline
           \textbf{SCST}~\cite{rennie2017self}       & $-$  & $34.2$ & $26.7$ & $55.7$ & $114.0$ & $-$   \\ \hline
           \textbf{LSTM-A}~\cite{yao2017boosting}   & $78.6$  & $35.5$ & $27.3$ & $56.8$ & $118.3$ & $20.8$   \\ \hline
           \textbf{StackCap}~\cite{gu2017stack}    & $78.6$  & $36.1$ & $27.4$ & $-$ & $120.4$ & $-$   \\ \hline
           \textbf{Up-Down}~\cite{anderson2018bottom}  & $79.8$ & $36.3$ & $27.7$ & $56.9$ & $120.1$ & $21.4$ \\ \hline
           \textbf{CAVP}~\cite{liu2018context}  & $-$& $38.6$ & $28.3$ & $58.5$ & $126.3$ & $21.6$ \\ \hline
           \textbf{GCN-LSTM$_{re}$}~\cite{yao2018exploring}  & $-$  & $-$ & $-$ & $-$ & $-$ & $-$ \\ \hline
           \textbf{GCN-LSTM$_{sem}$}~\cite{yao2018exploring}  & $80.5$  & $38.2$ & $28.5$ & $58.3$ & $127.6$ & $22.0$ \\ \hline
           \textbf{GCN-LSTM$_{fuse}$}~\cite{yao2018exploring} & $80.9$  & $38.3$ & $28.6$ & $58.5$ & $128.7$ & $22.1$ \\ \hline
           
\end{tabular}
}
\end{center}
\end{table}

\begin{table*}[t]
\begin{center}
\caption{The performances of our DC+GE and the compared methods, including ablative baselines and other state-of-the-art captioning methods, on online COCO testing set (\url{https://competitions.codalab.org/competitions/3221#results}). The metrics: B@N, M, R, C and S refer to BLEU@N, METEOR, ROUGE-L, CIDEr-D and SPICE respectively. In all cases, the scores are reported as percentage ($\%$)}
\label{table:tab_online}
\scalebox{0.93}{
\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		 %Model & \multicolumn{2}{|c|}{BLEU-1}  & \multicolumn{2}{|c|}{BLEU-2}  & \multicolumn{2}{|c|}{BLEU-3} & \multicolumn{2}{|c|}{BLEU-4} &\multicolumn{2}{|c|}{METEOR} &\multicolumn{2}{|c|}{ROUGE-L} & \multicolumn{2}{|c|}{CIDEr-D}\\ \hline
		 Model & \multicolumn{2}{|c|}{B@1}  & \multicolumn{2}{|c|}{B@2}  & \multicolumn{2}{|c|}{B@3} & \multicolumn{2}{|c|}{B@4} &\multicolumn{2}{|c|}{M} &\multicolumn{2}{|c|}{R-L} & \multicolumn{2}{|c|}{C-D}\\ \hline
		 Metric  &  c5 & c40 & c5 & c40 &  c5 & c40 & c5 & c40 & c5 & c40 & c5 & c40 & c5 & c40 \\ \hline
           %\textbf{OE}       & $76.8$ & $36.3$  & $27.3$ & $56.4$ & $114.3$  & $20.5$ & $79.9$ & $36.8$& $27.7$ & $57.0$ \\ \hline
           %\textbf{GE}       & $77.8$ & $36.3$  & $27.4$ & $56.6$ & $114.8$  & $20.5$ & $80.2$ & $37.1$& $27.6$ & $57.5$\\ \hline
           %\textbf{DC}       & $78.2$ & $36.4$  & $27.7$ & $56.7$ & $115.3$  & $20.7$ & $80.2$ & $37.5$& $28.0$ & $58.3$ \\ \hline
           \textbf{DC+GE}    & $80.6$ & $95.0$  & $65.0$ & $88.9$ & $50.1$  & $79.6$ & $37.8$ & $68.7$& $28.1$ & $37.0$ & $58.2$ & $73.1$ & $122.7$ & $125.5$\\ \hline 
           \textbf{DC+GE$_{fuse}$}    & $-$ & $-$  & $-$ & $-$ & $-$  & $-$ & $-$ & $-$& $-$ & $-$ & $-$ & $-$ & $-$ & $-$\\ \hline \hline
           \textbf{SCST}~\cite{rennie2017self}      & $78.1$ & $93.7$ & $61.9$ & $86.0$ & $47.0$ & $75.9$ & $35.2$ & $64.5$ & $27.0$ & $35.5$ & $56.3$ & $70.7$ & $114.7$ & $116.0$  \\ \hline
           \textbf{LSTM-A}~\cite{yao2017boosting}   & $78.7$ & $93.7$ & $62.7$ & $86.7$ & $47.6$ & $76.5$ & $35.6$ & $65.2$ & $27.0$ & $35.4$ & $56.4$ & $70.5$ & $116.0$ & $118.0$  \\ \hline
           \textbf{StackCap}~\cite{gu2017stack}     & $77.8$ & $93.2$ & $61.6$ & $86.1$ & $46.8$ & $76.0$ & $34.9$ & $64.6$ & $27.0$ & $35.6$ & $56.2$ & $70.6$ & $114.8$ & $118.3$   \\ \hline
           \textbf{Up-Down}~\cite{anderson2018bottom}    & $80.2$ & $95.2$ & $64.1$ & $88.8$ & $49.1$ & $79.4$ & $36.9$ & $68.5$ & $27.6$ & $36.7$ & $57.1$ & $72.4$ & $117.9$& $120.5$  \\ \hline
           \textbf{CAVP}~\cite{liu2018context}           & $80.1$ & $94.9$ & $64.7$ & $88.8$ & $50.0$ & $79.7$ & $37.9$ & $69.0$ & $28.1$ & $37.0$ & $58.2$ & $73.1$ & $121.6$& $123.8$    \\ \hline
            \textbf{GCN-LSTM$_{fuse}$}~\cite{yao2018exploring}           & $-$ & $-$ & $65.5$ & $89.3$ & $50.8$ & $80.3$ & $38.7$ & $69.7$ & $28.5$ & $37.6$ & $58.5$ & $73.4$ & $125.3$& $126.5$    \\ \hline
\end{tabular}
}
\end{center}
\end{table*}

\subsection{Enlightening Studies}
\textbf{Using Oracle Scene Graphs.}
In the sentence branch, the used sentence scene graphs are created by the ground truth captions. Then, suppose we have such kind of oracle scene graphs when inference, how better the generated captions can be? For exploring such a question, we generate sentence scene graphs by inputting the labeled captions, which belong to Karpathy's test set, into tools provided by~\cite{anderson2016spice}. Then we 1).directly feed the sentence graph embeddings to self-translator (route 1) to generate captions; 2).use sentence graph embeddings to consult the dictionary and then feed the consulted entries to self-translator (route 2) to generate captions. The results of different routes are shown in Table~\ref{table:tab_orac}. 

As we can see, the performances of using oracle sentence scene graphs (whether \textbf{Route 1} or \textbf{Route 2}) are far better than \textbf{DC+GE}. This is reasonable since the oracle sentence scene graphs contain almost no noises and are abundant in humans' descriptive expressions. By comparing \textbf{Route 1} and \textbf{Route 2}, we can see that directly using oracle sentence scene graphs would produce much better captions; and by comparing \textbf{Route 2} with \textbf{DC+GE}, we find that consulting dictionaries by oracle sentence scene graphs would generate more human-like captions. Both of these two observations encourage us to develop some more powerful techniques to compile and consult dictionary.

\begin{table}[t]
\begin{center}
\caption{The performances of using oracle sentence scene graphs}
\label{table:tab_orac}
\scalebox{0.88}{
\begin{tabular}{|c||c|c|c|c|c|c|}
		\hline
		   Metric   & B@1 & B@4 & M & R &  C & S\\ \hline
		   \textbf{DC+GE}    & $80.8$ & $38.4$ & $28.4$ & $58.6$ & $127.8$ & $21.8$\\ \hline
           \textbf{Route 1}  & $93.94$ & $65.21$& $38.51$ & $71.85$ & $177.0$ & $34.38$\\ \hline
           \textbf{Route 2}  & $90.38$ & $53.86$& $34.03$ & $66.53$ & $153.2$ & $30.69$\\ \hline
\end{tabular}
}
\end{center}
\end{table}

\textbf{Using Web Description Texts.}
There is a nearly unlimited amount of free description texts available in website, thus, if these resources can be rationally exploited, the performance of captioning model will naturally be improved. For discovering the potential ability of using web description texts in our model, we use the texts provided by Visual Genome~\cite{krishna2017visual} instead of COCO caption dataset~\cite{lin2014microsoft} to learn the dictionary in sentence branch. And then we follow route 3 to train image branch. The results is demonstrated in~\ref{table:tab_web}.
\begin{table}[t]
\begin{center}
\caption{The performances of using web description texts}
\label{table:tab_web}
\scalebox{0.95}{
\begin{tabular}{|c||c|c|c|c|c|c|}
		\hline
		   Metric   & B@1 & B@4 & M & R &  C & S\\ \hline
		   \textbf{OE}       & $79.9$ & $36.8$& $27.7$ & $57.0$ & $120.6$ & $20.9$\\ \hline
		   \textbf{Web}  & $-$ & $-$& $-$ & $-$ & $-$ & $-$\\ \hline
		   \textbf{DC+GE}    & $80.8$ & $38.4$ & $28.4$ & $58.6$ & $127.8$ & $21.8$\\ \hline
          
\end{tabular}
}
\end{center}
\end{table}

==> intro.tex <==
%%%%%%%%% BODY TEXT
\section{Introduction}
For image captioning, there are two ingredients spurring its success: a visual system, which used as encoding module, should be able to accurately recognize the appeared visual clues; and one language system, which used as decoding module, should be able to compose these revealed clues to one human-like caption.

On the one hand, benefiting from the ingeniously designed deep networks, some fundamental computer vision tasks like classification, detection or segmentation have achieved unprecedented success. 
The fruits of these achievements are further extended to the image captioning task that these deep CNNs are usually used as encoding module to extract representations which are rich in visual clues.
For example, by exploiting a well pre-trained object detection network, Faster R-CNN~\cite{ren2015faster}, to seek the salient regions in one image, the generated captions now are more visual grounding to the images~\cite{anderson2018bottom}. Here, visual grounding means that the named concepts in one caption are associated to the objects appeared in one image~\cite{lu2018neural}.

On the another hand, in order to capture the intimate connection among a sentence, Long Short Term Memory (LSTM)~\cite{hochreiter1997long} is usually built as one decoding module to generate the caption. 
Also, for the sake of establishing closer ties between generated language with images, attention mechanisms of different usage~\cite{xu2015show,lu2017knowing,anderson2018bottom} are incorporated into the decoding systems. Though these mechanisms own diverse scheming details, the main role are similar that try to make the decoding module focus on some specific regions of the image conditioned on the sentence generated so far.
Furthermore, by applying reinforcement learning~\cite{rennie2017self} to optimize the whole system with sentence-level metric such as CIDEr metric~\cite{vedantam2015cider}, the generated captions are more likely to be fluent, well-formed compared with the system trained by cross-entropy loss.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth,trim = 5mm 3mm 5mm 5mm,clip]{latex/fig_intro.pdf}
   \caption{}
\label{fig:fig_intro}
\end{figure}

However, generating grounding and fluent captioning is only one small step in the long march of generating human-like caption. For one image, humans can not only recognize the salient objects along with their visual attributes (\ie colour, shape or size) to compose one description, but also associate these visual cues to some more complex or descriptive terms by common sense and life experiences. For example, as shown in Fig~\ref{fig:fig_intro}, human may describe `yellow banana' as `ripe banana' or describe `a room full with many items' as `cluttered room'. 

While some modern systems like~\cite{anderson2018bottom,lu2018neural} can hardly compose one caption with these descriptive or more human-like terms. There are two reasons which cause the model be difficult in capturing these more flexible terms.
1). These models usually use object-level embedding, \eg the RoI pooling of one object. Then, when generating next word, the language model usually only focuses on one object by predicting one attention distribution over these objects. Such object-level hinder the system from composing complex phrases since these kind of embeddings usually only contain the information about the categories of these objects or at most some additional visual attribute information. 
2). The second reason is that these systems are usually optimized by CIDEr, which is a consensus-based evaluation protocol that it prefers a description which owns more similarity to the majority reference captions. Then the caption system trends to provide overly general captions which only combines the appeared salient objects together as one grounding and fluent caption, while suppress the various and flexible descriptions about interesting details appeared in one image. 

For generating more human-like captions, we propose a captioning model which is trained by `Dictionary Compiling and Consulting' strategy. For `Dictionary Compiling', firstly, we use graph neural network to embed one sentence scene graph to sentence embeddings and recompose one sentence from these embeddings with a self-translator. In this stage, the sentence graph neural network and self-translator are trained. Then we compile one dictionary which should save these sentence embeddings. When compiling dictionary, we use these sentence embeddings as indexes to consult entries from the dictionary, and then feed these consulted entries into the self-translator to recompose the sentence. After compiling the dictionary, when generating one caption from one image, we use one image graph neural network to embed visual feature and then use them to consult the compiled dictionary to find corresponding entries. And the consulted entries and these visual embedding features are all feed into one caption generator to get the final caption. Here we use a differentiable operation to implement consulting, and thus the whole system can be trained end-to-end.

Compared with object-level embedding used in~\cite{lu2017knowing,lu2018neural,anderson2018bottom}, we use graph neural network to embed the triplet information like <subject-predicate-object> or <attribute-object> together. From the language perspective, object-level embedding corresponding to word-level expression and graph-level embedding corresponding to phrase-level expression.
By using attention mechanism to predict an attention distributions over these graph embeddings, the language system can incorporate more visual clues. Furthermore, the visual graph embedding is used to consult corresponding dictionary entries which contains abundant distinctive expressions. Both visual graph embedding and the consulted dictionary entries enable the language system to generate more human-like sentences.  

\textbf{Contributions:} Our contributions can be concluded as follows:
\begin{itemize}[nolistsep]
\item We propose the Dictionary Compiling and Consulting model, which can incorporate visual embeddings with more clues and phrase embeddings with distinctive expressions together to compose more human-like captions.
\item Graph neural network is used to embed scene graph information together to get graph-level embedding for image and sentence.
\item A dictionary which contains embeddings with abundant human-like expressions is compiled. When generating captions, this dictionary is consulted with visual graph embeddings as indexes to provide more complex and descriptive information for composing human-like descriptions.
\item Exhaust experiments show that our proposed method can achieve obvious improvements compared with baselines. Ablation studies are also designed to prove that each added component play certain roles in improving performance. 
\end{itemize}
